An Elementary Introduction to Kalman Filtering

Kalman filtering is a classic state estimation technique used in application areas such as signal processing and autonomous control of vehicles. It is now being used to solve problems in computer systems such as controlling the voltage and frequency of processors. Although there are many presentations of Kalman filtering in the literature, they usually deal with particular systems like autonomous robots or linear systems with Gaussian noise, which makes it difficult to understand the general principles behind Kalman filtering. In this paper, we first present the abstract ideas behind Kalman filtering at a level accessible to anyone with a basic knowledge of probability theory and calculus, and then show how these concepts can be applied to the particular problem of state estimation in linear systems. This separation of concepts from applications should make it easier to understand Kalman filtering and to apply it to other problems in computer systems.

==> kalmanfilter.tex <==
Sections~\ref{sec:scalar} and Section~\ref{sec:vector} explain the generic problem of data fusion using an optimal linear estimator. In this section, we discuss \kfs which is a popular data fusion technique in the field of information theory~\cite{kalman-techreport}. The core steps of the \kf algorithm can be easily understood from the ideas discussed in earlier sections.

The \kf algorithm was proposed by Rudolf E. K\'{a}lm\'{a}n in 1960~\cite{kalman-filter}, more than fifty years ago. It is used to fuse multiple estimates of a system state, ``filtering'' out noisy data. % The term ``filter'' is used to indicate that the process of finding the optimal estimate from noisy data amounts to ``filtering out'' the noise.
The algorithm fuses a series of \emph{observed} measurements with \emph{estimates} over time, and produces estimates of unknown variables such as the system state. Note that \emph{both} the measurement and the estimate can contain statistical noise.

The \kf algorithm is recursive and operates in a time-step manner. The two steps in the algorithm are: \emph{prediction} and \emph{update}. At time $t_{i}$, the prediction step estimates the current state of the variables based on prior observations till $t_{i-1}$. Once the measurement at time $t_{i}$ is available, the algorithm merges the potentially noisy measurement data with the estimate using a \emph{weighted} average. Intuitively, observations with higher confidence are given more weight. \Kfs are typically presented as a linear dynamic system  of equations that minimize the mean square error (\mse) of the system (~Appendix~\ref{sec:defmse}), and hence are also known as the Linear Quadratic estimation algorithm~\cite{xx}.

The success of \kfs is due to its small computational requirement and stochastical properties. This allows the filter to average over a lot of data, effectively hiding any outliers and zero in on the optimal linear estimator. For example, the \kf does not make any assumptions about the nature of the error---the errors need not be Gaussian. However, it has been proved that \kfs are the optimal linear estimators in cases where the errors are indeed Gaussian or the models perfectly match the real applications. As such \kfs have been applied to multiple application domains such as global positioning systems, motion planning in robotics, and signal processing, and even in safety-critical domains like autonomous navigation.

% Kalman filter is an algorithm that fuses a series of measurements observed with estimates over time, containing statistical noise and other inaccuracies, and produces estimates of unknown variables.

% \swarnendu{Francis, I think we should separate the description of Kalman Filters from the example. Let us just talk about KF in prose in the above paragraph. Then, we can give one or more examples as a separate Subsection.}
% \francis{1. I guess the intro of KF will be introduced in the first secton? 2. I will modify notations later}

\subsection{Understanding KF with a 1-D example}
\label{sec:simple_exp}

%\begin{figure}[!ht]
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{images/car_example2.png}
    \caption{1-D car example}
    \label{fig:car_example}
\end{figure}

\iffalse
The formulation of this problem is given in Equations~\ref{eqn:nextesitmate} and \ref{eqn:nextobservation}.
\begin{align}
\label{eqn:fuse}
x_{t+1|t+1} &= Fuse(x_{t+1|t}, z_{t+1})
\end{align}
\fi

In Figure~\ref{fig:car_example}, we use a simple 1-D car motion example to demonstrate one time step of the \kf algorithm. The example assumes that a car is running along the railway. To keep the problem simple, we define the distance between the car and the anchor on the left as the only component in the state vector, denoted as $x_{t|t}$, with variance $\sigma^2_{t|t}$ representing the uncertainty.
In addition, assume that control signals to the car make the car move at some constant velocity, denoted as $u_t$ in Figure~\ref{fig:car_example}.
These simplifications may not represent reality, for example, the velocity may vary during the car motion. Therefore, a \emph{random noise} $w_t$ with variance $R_t$ is assumed.
Given Equation \ref{eqn:nextesitmate}, an estimate of the distance at time step $t+1$ is obtained during the prediction step of the \kf, denoted as $x_{t+1|t}$, with variance $\sigma^2_{t|t} + R_t$.
\begin{align}
\label{eqn:nextesitmate}
%x_{t+1|t} &= F_tx_{t|t} + B_tu_t + w_t
x_{t+1|t} &= x_{t|t} + u_t*1 + w_t
\end{align}

An observation is made during the update step of the \kf based on the car's state at time $t+1$. Again to keep the example simple, we assume that we observe the distance directly (sometimes we may not be able to observe the result directly).
% \swarnendu{Francis: what does the previous statement mean?}
However, the observation may have some uncertainty as well.
Therefore, $v_{t+1}$, another \emph{random noise} vector, is added to obtain the observation vector $z_{t+1}$ at time $t+1$, with variance $Q_t$. $z_{t+1}$ is obtained as shown in Equation \ref{eqn:nextobservation}
\begin{align}
\label{eqn:nextobservation}
%z_{t+1} &= H_tx_{t+1|t} + v_{t+1} \\
z_{t+1} &= x_{t+1|t} + v_{t+1}
\end{align}

Now we have an estimates and an observation, which are uncorrelated.
The final step is to fuse $x_{t+1|t}$ and $z_{t+1}$ to get $x_{t+1|t+1}$ and $\sigma^2_{t+1|t+1}$, as mentioned in previous sections.

Intuitively, the above process is shown in Fig. \ref{fig:one_step_simple}. The key insight here is that before the execution of time $t+1$, we have an optimal estimate $x_{t|t}$ with variance $\sigma^2_{t|t}$, and a new optimal estimate $x_{t+1|t+1}$ with variance $\sigma^2_{t+1|t+1}$ can be obtained after the one time step execution. To be specific, a new estimate at time $t+1$ is made on the basis of $x_{t|t}$ and control signal $u_t$. A new observation is also made at time $t+1$. The fusion of this new estimate and this new observation is the optimal estimate of time $t+1$, with updated uncertainty $\sigma^2_{t+1|t+1}$.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{images/one_step_simple.png}
    \caption{One time step of the car motion example}
    \label{fig:one_step_simple}
\end{figure}

\subsection{Understanding KF with a 2-D example}
\label{sec:standard_exp}

In this section, we will extend the simplified 1-D car motion to a multi-dimensional problem. We define the car's state to be a vector of the car's distance from the anchor and the velocity, denoted as $\kvec{x}_{t|t} = (d, v)^T$, with covariance matrix $\pmb{\Sigma}_{t|t}$. If the railway is smooth, the velocity of the car will be a constant and the distance will increase linearly. This part of the movement is given by $\kmat{F}_t$, which can be represented by $[\begin{smallmatrix} 1&1\\ 0&1 \end{smallmatrix}]$. In reality, the railway will have some resistance, resulting in loss of velocity. We say that the resistance is the control signal, denoted as $\kvec{u}_t$. Therefore, the state vector needs correction---$\kmat{B}_t$ transforms the resistance into velocity and distance correction.

A \emph{random noise}  vector $\kvec{w}_t$, with covariance matrix $\kmat{R}_t$, is also considered. The state estimate expression is given in Equation~\ref{eqn:nextesitmate_value}.
\begin{align}
\label{eqn:nextesitmate_value}
\kvec{x}_{t+1|t} &= \kmat{F}_t\kvec{x}_{t|t} + \kmat{B}_t\kvec{u}_t + \kvec{w}_t\nonumber\\
\end{align}

In addition, the way to update covariance matrix is also different. The covariance matrix of $\kvec{x}_{t|t}$ applies the $\kmat{F}_t$ transformation before adding to $\kmat{R}_t$, as shown in Equation~\ref{eqn:nextesitmate_covariance}.
\begin{align}
\label{eqn:nextesitmate_covariance}
\pmb{\Sigma}_{1} &= \kmat{F}_t \pmb{\Sigma}_{t|t} \kmat{F}^T + \kvec{R}_t
\end{align}

Often, not all the states in the state vector are easily measurable. For example, the distance may be easy to measure but the velocity is not if a velocity measurement device is not available. The measurement expression is given in Equation~\ref{eqn:nextobservation_standard}, where $\kmat{H}_{t+1}$ can be $[\begin{smallmatrix} 1&0 \end{smallmatrix}]$ if only the distance is observable. $\kvec{v}_{t+1}$ is a random noise vector whose length is one in this case, with variance $\kmat{Q}_{t+1}$.
\begin{align}
\label{eqn:nextobservation_standard}
\kvec{z}_{t+1} &= \kmat{H}_{t+1}\kvec{x}_{t+1|t} + \kvec{v}_{t+1} \\
\label{eqn:nextobservation_covariance}
\pmb{\Sigma}_{2} &= \kmat{Q}_{t+1}
\end{align}

Figure~\ref{fig:one_step} shows how this example works. The procedure is similar to Figure~\ref{fig:one_step_simple}, except that the covariance part needs a linear transformation.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{images/one_step.png}
    \caption{One time step of the car motion example}
    \label{fig:one_step}
\end{figure}

Now it's the time to apply Equation~\ref{eqn:M0}. However, note that $\pmb{\Sigma}_1$ and $\pmb{\Sigma}_2$ are describing different things, even in different dimensions. $\pmb{\Sigma}_1$ describes the covariance of $\kvec{x}_{t+1|t}$ while $\pmb{\Sigma}_2$ describes the variance of $\kvec{z}_{t+1}$. In addition, $\kvec{z}_{t+1}$ is the result of applying $\kmat{H}_{t+1}$ to $\kvec{x}_{t+1|t}$. Hence, before applying Equation~\ref{eqn:M0}, $\kmat{H}_{t+1}$ should also be applied to $\pmb{\Sigma}_1$ when adding to $\kmat{Q}_{t+1}$. The standard expression for Kalman Gain $\kmat{K}_{t+1}$ is given in Equation~\ref{eqn:standard_K}. Note that $\kmat{H}_{t+1}$ is also applied to the numerator since we are only observing distance, only the variance of distance and the covariance of distance and velocity should be utilized.

\begin{align}
\label{eqn:standard_K}
\kmat{K}_{t+1} &= \frac{\pmb{\Sigma}_1 \kmat{H}^T_{t+1}}{\kmat{H}_{t+1} \pmb{\Sigma}_1\kmat{H}^T_{t+1} + \kmat{Q}_{t+1}}
\end{align}

The fusion result is given in Equation~\ref{eqn:standard_x} and Equation~\ref{eqn:standard_sigma} in terms of $\kmat{K}_{t+1}$. The distance and velocity components in $\kvec{x}_{t+1|t+1}$ is corrected by distance difference and distance-speed covariance. The covariance matrix part is updated accordingly.
\begin{align}
\label{eqn:standard_x}
\kvec{x}_{t+1|t+1} &= \kvec{x}_{t+1|t} + \kmat{K}_{t+1}(\kvec{z}_{t+1} - \kmat{H}_{t+1}\kvec{x}_{t+1|t}) \\
\label{eqn:standard_sigma}
\pmb{\Sigma}_{t+1|t+1} &= (\pmb{I} - \kmat{K}_{t+1}\kmat{H}_{t+1})\pmb{\Sigma}_{1}
\end{align}

\subsection{Car motion example experiment result}
\label{sec:car_result}

We will now use the above setup to show how \kfs are able to predict the state using a concrete example. As before, the state of the car is a vector of the velocity and the distance.
% Using the above setup, we will show that \kf does a good job in estimating distance and velocity.
Let us assume that the car starts at distance $10m$ with an initial  velocity of $20m/s$. The resistance of the ground cause a $-2m/s^2$ acceleration. The time step used in Fig.~\ref{fig:car_motion_result} is $0.025s$. The variance of distance observation is $20$ and and the covariance of one estimation is $[\begin{smallmatrix} 4&0 \\ 0&4 \end{smallmatrix}]$. In Fig.~\ref{fig:car_motion_result}, we show the simulation data of distance in the first 10 seconds. We can see that \kf did a good job in eliminate the noise and made the optimal choice.

\francis{I know this part need much update, so I make it simple for now.}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{images/car_motion_result.pdf}
    \caption{The car motion example result}
    \label{fig:car_motion_result}
\end{figure}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

